A Catalog of Enumeration Formulas for Bouquet and Dipole Embeddings Under Symmetries

Motivated by a problem arising out of DNA origami, we give a general counting framework and enumeration formulas for various cellular embeddings of bouquets and dipoles under different kinds of symmetries. Our algebraic framework can be used constructively to generate desired symmetry classes, and we use Burnside's Lemma with various symmetry groups to derive the enumeration formulas. Our results assimilate several existing formulas into this unified framework. Furthermore, we provide new formulas for bouquets with colored edges (and thus for bouquets in nonorientable surfaces) as well as for directed embeddings of directed bouquets. We also enumerate vertex-labeled dipole embeddings. Since dipole embeddings may be represented by permutations, the formulas also apply to certain equivalence classes of permutations and permutation matrices. The resulting bouquet and dipole symmetry formulas enumerate structures relevant to a wide variety of areas in addition to DNA origami, including RNA secondary structures, Feynman diagrams, and topological graph theory. For uncolored objects we catalog 58 distinct sequences, of which 43 have not, as far as we know, been described previously.

==> countbib.tex <==
% Problem is that MDPI/Symmetry files do not put references in
% alphabetical order by author; they put them in order of occurrence.

% Created by running MDPI/Symmetry shell using count.bib, then
% reordering items in count.bbl in order of bibliography created by
% Elsevier's .bst file.


\begin{thebibliography}{999}

\bibitem[Andersen \em{et~al.}(1996)Andersen, Mattes, and Reshetikhin]{AMR96}
Andersen, J.; Mattes, J.; Reshetikhin, N.
\newblock The Poisson structure on the moduli space of flat connections and
  chord diagrams.
\newblock {\em Topology} {\bf 1996}, {\em 35},~1069--1083.
\newblock {\url{https://doi.org/10.1016/0040-9383(95)00059-3}}.

\bibitem[Bon \em{et~al.}(2008)Bon, Vernizzi, Orland, and Zee]{Bon08}
Bon, M.; Vernizzi, G.; Orland, H.; Zee, A.
\newblock Topological Classification of {RNA} Structures.
\newblock {\em J. Mol. Biol.} {\bf 2008}, {\em 379},~900--911.

\bibitem[Chen \em{et~al.}(2018)Chen, Gao, and Huang]{CGH18}
Chen, Y.; Gao, X.; Huang, Y.
\newblock Enumerating unlabelled embeddings of digraphs.
\newblock {\em Canad. Math. Bull.} {\bf 2018}, {\em 61},~55--69.
\newblock {\url{https://doi.org/10.4153/CMB-2017-050-9}}.

\bibitem[Ellingham and Ellis-Monaghan(2019)]{EE-M19}
Ellingham, M.N.; Ellis-Monaghan, J.A.
\newblock Edge-outer graph embedding and the complexity of the {DNA} reporter
  strand problem.
\newblock {\em Theoret. Comput. Sci.} {\bf 2019}, {\em 785},~117--127.
\newblock {\url{https://doi.org/10.1016/j.tcs.2019.03.019}}.

\bibitem[Ellis-Monaghan and Moffatt(2013)]{E-MM13}
Ellis-Monaghan, J.; Moffatt, I.
\newblock {\em Graphs on surfaces: twisted duality, polynomials and knots};
  SpringerBriefs in Mathematics,  2013.

\bibitem[Ellis-Monaghan \em{et~al.}(2017)Ellis-Monaghan, Pangborn, Seeman,
  Blakeley, Disher, Falcigno, Healy, Morse, and Singh]{E+17}
Ellis-Monaghan, J.; Pangborn, G.; Seeman, N.; Blakeley, S.; Disher, C.;
  Falcigno, M.; Healy, B.; Morse, A.; Singh, B.~Westland, M.
\newblock Design Tools For Reporter Strands and {DNA} Origami Scaffold Strands.
\newblock {\em Theoret. Comput. Sci.} {\bf 2017}, {\em 671},~69--78.

\bibitem[Ellis-Monaghan \em{et~al.}(2015)Ellis-Monaghan, McDowell, Moffatt, and
  Pangborn]{E+15cost}
Ellis-Monaghan, J.; McDowell, A.; Moffatt, I.; Pangborn, G.
\newblock {DNA} origami and the complexity of Eulerian circuits with turning
  costs.
\newblock {\em Natural Computing} {\bf 2015}, {\em 14},~491--503.

\bibitem[Feng \em{et~al.}(2010)Feng, Kwak, and Zhou]{FKZ10}
Feng, Y.Q.; Kwak, J.H.; Zhou, J.X.
\newblock Congruence classes of orientable 2-cell embeddings of bouquets of
  circles and dipoles.
\newblock {\em Electron. J. Combin.} {\bf 2010}, {\em 17},~Research Paper 41,
  15.

\bibitem[Feng \em{et~al.}(2013)Feng, Kwak, and Zhou]{FKZ13}
Feng, Y.; Kwak, J.H.; Zhou, J.
\newblock Enumerating reflexible 2-cell embeddings of connected graphs.
\newblock {\em Sci. China Math.} {\bf 2013}, {\em 56},~933--950.
\newblock {\url{https://doi.org/10.1007/s11425-012-4544-2}}.

\bibitem[Furst \em{et~al.}(1989)Furst, Gross, and Statman]{FGS89}
Furst, M.L.; Gross, J.L.; Statman, R.
\newblock Genus distributions for two classes of graphs.
\newblock {\em J. Combin. Theory Ser. B} {\bf 1989}, {\em 46},~22--36.
\newblock {\url{https://doi.org/10.1016/0095-8956(89)90004-X}}.

\bibitem[Gross and Furst(1987)]{GF87}
Gross, J.L.; Furst, M.L.
\newblock Hierarchy for imbedding-distribution invariants of a graph.
\newblock {\em J. Graph Theory} {\bf 1987}, {\em 11},~205--220.
\newblock {\url{https://doi.org/10.1002/jgt.3190110211}}.

\bibitem[Gross \em{et~al.}(1989)Gross, Robbins, and Tucker]{GRT89}
Gross, J.L.; Robbins, D.P.; Tucker, T.W.
\newblock Genus distributions for bouquets of circles.
\newblock {\em J. Combin. Theory Ser. B} {\bf 1989}, {\em 47},~292--306.
\newblock {\url{https://doi.org/10.1016/0095-8956(89)90030-0}}.

\bibitem[Gross and Tucker(2001)]{GT}
Gross, J.L.; Tucker, T.W.
\newblock {\em Topological graph theory}; Dover Publications, Inc. Mineola, NY,
   2001; pp. xvi+361.
\newblock Reprint of the 1987 original [Wiley, New York; MR0898434 (88h:05034)]
  with a new preface and supplementary bibliography.

\bibitem[Kim and Park(2000)]{KP00}
Kim, J.H.; Park, Y.K.
\newblock Incongruent embeddings of a bouquet into surfaces.
\newblock {\em Bull. Austral. Math. Soc.} {\bf 2000}, {\em 61},~89--96.
\newblock {\url{https://doi.org/10.1017/S0004972700022048}}.

\bibitem[Krzywinski \em{et~al.}(2009)Krzywinski, Schein, Birol, Connors,
  Gascoyne, Horsman, and Marra]{Circos09}
Krzywinski, M.I.; Schein, J.E.; Birol, I.; Connors, J.; Gascoyne, R.; Horsman,
  D.; Marra, S.J.J.M.A.
\newblock Circos: An information aesthetic for comparative genomics.
\newblock {\em Genome Res.} {\bf 2009}, {\em 19},~1639--45.

\bibitem[Kwak and Lee(1994)]{KL94}
Kwak, J.H.; Lee, J.
\newblock Enumeration of graph embeddings.
\newblock {\em Discrete Math.} {\bf 1994}, {\em 135},~129--151.
\newblock {\url{https://doi.org/10.1016/0012-365X(93)E0075-F}}.

\bibitem[Mohar and Thomassen(2001)]{MT}
Mohar, B.; Thomassen, C.
\newblock {\em Graphs on surfaces}; Johns Hopkins Studies in the Mathematical
  Sciences, Johns Hopkins University Press, Baltimore, MD,  2001; pp. xii+291.

\bibitem[Mull(1999)]{Mul99}
Mull, B.P.
\newblock Enumerating the orientable {$2$}-cell imbeddings of complete
  bipartite graphs.
\newblock {\em J. Graph Theory} {\bf 1999}, {\em 30},~77--90.
\newblock
  {\url{https://doi.org/10.1002/(SICI)1097-0118(199902)30:2<77::AID-JGT2>3.3.CO;2-N}}.

\bibitem[Mull \em{et~al.}(1988)Mull, Rieper, and White]{MRW88}
Mull, B.P.; Rieper, R.G.; White, A.T.
\newblock Enumerating {$2$}-cell imbeddings of connected graphs.
\newblock {\em Proc. Amer. Math. Soc.} {\bf 1988}, {\em 103},~321--330.
\newblock {\url{https://doi.org/10.2307/2047573}}.

\bibitem[nLa()]{nLab}
{nLab} chord diagram page.
\newblock \url{https://ncatlab.org/nlab/show/chord+diagram}.
\newblock Accessed: 2022-04-25.

\bibitem[OEI()]{OEIS}
OEIS Foundation Inc. (2022), The On-Line Encyclopedia of Integer Sequences,.
\newblock Published electronically at \url{http://oeis.org}.
\newblock Accessed: 2022-05-25.

\bibitem[Pelesko(2007)]{Pel07}
Pelesko, J.
\newblock {\em Self Assembly: The Science of Things That Put Themselves
  Together}; Taylor \& Francis Group, LLC,  2007.

\bibitem[Penner(2016)]{Pen16}
Penner, R.C.
\newblock Moduli spaces and macromolecules.
\newblock {\em Bull. Amer. Math. Soc. (N.S.)} {\bf 2016}, {\em 53},~217--268.
\newblock {\url{https://doi.org/10.1090/bull/1524}}.

\bibitem[Rieper(1990)]{Rie90}
Rieper, R.G.
\newblock The enumeration of graph imbeddings.
\newblock Ph.D. dissertation, Western Michigan University,  1990.

\bibitem[Rothemund(2006)]{Rot06}
Rothemund, P.W.
\newblock Folding {DNA} to create nanoscale shapes and patterns.
\newblock {\em Nature} {\bf 2006}, {\em 440},~297--302.

\bibitem[Seeman(2016)]{S15}
Seeman, N.C.
\newblock {\em Structural {DNA} Nanotechnology}; Cambridge University Press,
  2016.

\bibitem[Stahl(1983)]{Sta83}
Stahl, S.
\newblock Average genus of classes of graph embeddings.
\newblock {\em Congr. Numer.} {\bf 1983}, {\em 40},~375--388.

\bibitem[Veneziano \em{et~al.}(2016)Veneziano, Ratanalert, Zhang, Zhang, Yan,
  Chiu, Bathe, et~al.]{V+16}
Veneziano, R.; Ratanalert, S.; Zhang, K.; Zhang, F.; Yan, H.; Chiu, W.; Bathe,
  M.;  et~al.
\newblock Designer Nanoscale {DNA} Assemblies Programmed from the Top Down.
\newblock {\em Science} {\bf 2016}.
\newblock {\url{https://doi.org/10.11.26/science.aaf4388}}.

\bibitem[Wu \em{et~al.}(2009)Wu, Jonoska, and Seeman]{WJS09}
Wu, G.; Jonoska, N.; Seeman, N.C.
\newblock Construction of a {DNA} nano-object directly demonstrates
  computation.
\newblock {\em Biosystems} {\bf 2009}, {\em 98},~80 -- 84.
\newblock
  {\url{https://doi.org/10.1016/j.biosystems.2009.07.004}}.

\bibitem[Xuong(1979{\natexlab{a}})]{Xuo79b}
Xuong, N.H.
\newblock How to determine the maximum genus of a graph.
\newblock {\em J. Combin. Theory Ser. B} {\bf 1979}, {\em 26},~217--225.
\newblock {\url{https://doi.org/10.1016/0095-8956(79)90058-3}}.

\bibitem[Xuong(1979{\natexlab{b}})]{Xuo79a}
Xuong, N.H.
\newblock Upper-embeddable graphs and related topics.
\newblock {\em J. Combin. Theory Ser. B} {\bf 1979}, {\em 26},~226--232.
\newblock {\url{https://doi.org/10.1016/0095-8956(79)90059-5}}.

\bibitem[Zaj\k{a}c \em{et~al.}(2018)Zaj\k{a}c, Geary, Andersen,
  Dabrowski-Tumanski, Su\l{}kowska, and Sulkowski]{Zaj+18}
Zaj\k{a}c, S.; Geary, C.; Andersen, E.S.; Dabrowski-Tumanski, P.; Su\l{}kowska,
  J.I.; Sulkowski, P.
\newblock Genus trace reveals the topological complexity and domain structure
  of biomolecules.
\newblock {\em Sci. Rep.} {\bf 2018}, {\em 8},~17537.

\end{thebibliography}

